Quotient-Space Motion Planning

A motion planning algorithm computes the motion of a robot by computing a path through its configuration space. To improve the runtime of motion planning algorithms, we propose to nest robots in each other, creating a nested quotient-space decomposition of the configuration space. Based on this decomposition we define a new roadmap-based motion planning algorithm called the Quotient-space roadMap Planner (QMP). The algorithm starts growing a graph on the lowest dimensional quotient space, switches to the next quotient space once a valid path has been found, and keeps updating the graphs on each quotient space simultaneously until a valid path in the configuration space has been found. We show that this algorithm is probabilistically complete and outperforms a set of state-of-the-art algorithms implemented in the open motion planning library (OMPL).

==> path-space-decomposition.tex <==
\section{Decomposition of Path Space}

We will impose the following assumptions onto the problem
\begin{enumerate}
  \item Make/Break only one contact at a time
  \item Contacts only at specific pressure points, prespecified on the robot's body.
  \item Contacts are non-slipping
  \item Robot is in Static Equilibrium
\end{enumerate}

We like to decompose the path space hierarchically based on necessary
conditions. Our idea is to impose necessary conditions on the path space to
split it into smaller spaces. We do this procedure on different levels. For each
level we develop cost functions to compare different subspaces with each other.
This will create a hierarchical motion graph, where each node is a path subspace
and each edge is an inclusion relation. The union of nodes on the same level should
ideally compose the whole path space.

For motion planning, the idea is to quickly traverse the graph and move down
until we reach a lowest subspace. Then we start planning in this low-dimensional
subspace until we either find a solution or we backtrack back the graph.

We start from the very beginning: A path is feasible if it is
continuous. A continuous path is com-feasible if the center of mass is 'near' the
environment and the environment is directed 'against' the force field. A
com-feasible path is contact-feasible if...

\subsection{Center of Mass Path Space}

\begin{equation}
  \begin{aligned}
    \PSC &= \PS /_{\simeq_C}\\
  \end{aligned}
\end{equation}

which is the quotient space of $\PS$ under the equivalence relation $\simeq_C =
\{ \path,\path' \in \PS\ |\ \com(\path) \simeq \com(\path')\}$.

It is important to introduce high-level feasibility conditions on the path
space. We use two necessary conditions for feasibility: the reachability
condition \cite{tonneau_2016} and force field constraint. If the path obeys the
necessary conditions, we call the path com-feasible.

\subsubsection{Planning with Reachability Condition}

As remarked by \cite{tonneau_2016}, a path in $\PSC$ needs to have the
reachability property: it is feasible if it is near the environment such that
contacts can be made, but not too near such that the body is not in collision.
One way to accomplish that is to introduce two swept-volume approximations, an
inner and an outer one. 

\def\sin{\ensuremath{S_I}}
\def\sout{\ensuremath{S_O}}

We like to search $\PSC$ by growing a sphere $\sout$ with a sphere $\sin$ inside. The radius
of $\sin$ is equal to the maximum sphere included in a rigid body of the robot
(over all rigid bodies). If all bodies are represented by convex polygons, then
this can be solved by convex optimization using the maximum circle included in
convex polygon \cite{boyd}.

The radius of the outer sphere $\sout$ can be found by randomly sampling
configurations and taking the maximum sphere which encompasses the swept volume.

Motion planning for the sphere can be done by sampling positions in $\R^3$,
checking that $\sin$ is collision free, and checking that $\sout$ is \emph{in
collision}.

We note that the reachability condition can be backtraced to the decomposition
based planning \cite{brock_2001} where spheres are sampled to approximate the collision free
workspace of the robot. See also \cite{rickert_2014}.

We have visualized an approximation of the path space of the center of mass in
Figure \ref{fig:spider}.


\subsubsection{Planning with Force Field Constraint}

A path in $\PSC$ obeying the reachability condition might be infeasible
because none of the contact surfaces is oriented against the force field in the
environment. Imagine a ceiling and a gravity force field. Contacts on the
ceiling can produce ground-reaction forces only in the gravity direction, and
are therefore not helpful for static stability. 

In a second stage, we propose to further cut spheres by introducing a direction:
We cut the outer sphere into half, in the direction perpendicular to the
direction of the acting force field. For example perpendicular to the gravity
force vector. We call the part in the direction of the force field vector the
lower half and denote it by $S_{o,L}$. $S_{o,L}$ needs to be in collision
\footnote{TODO: this will disallow motions where the hand is grasping a
horizontal ladder for example, making it not a necessary condition anymore}

This will eliminate spheres which are near ceilings in a gravity field for example.

\subsection{Contact Path Space}

Let $\{r_0,\cdots,r_K\}$ be a set of contacts points on the robot's body, and
let $\env$ be the set of obstacle regions in $\R^3$. Each
contact point has an associated distance function $d(r_k,\env)$, which measures the
distance between $r_k$ and the environment $\env$. A contact point is said to be
in contact iff $d(r_k,\env)=0$.

This distance function decomposes the path space: For each $r_k$, we have the
path space

\begin{equation}
  \begin{aligned}
    \PSK &= \{ \path \in \PSC\ |\ d(r_k,\env)=0 \}
  \end{aligned}
\end{equation}

Since contacts do not slip, this space is foliated \footnote{A p-dimensional foliation of an n-manifold $\M$ is a collection
  $\{\M_\alpha\}$ of pairwise disjoint, connected, immersed p-dimensional submanifolds of
$\M$, such that its union $\cup \M_\alpha = \M$ \cite{lee_2003}.} indexed by $e \in \env$. Each
leave of the foliation is of the form
\begin{equation}
  \begin{aligned}
    \PSKE &= \{ \path \in \PSC\ |\ d(r_k,e)=0 \}
  \end{aligned}
\end{equation}

A path through $\PSKE$ can be thought of as a path through the space of inverse
kinematic solutions while keeping the contact point $r_k$ fixed. 

A path of a robot in static equilibrium needs to be a piecewise sequence of
paths in $\PSK$, for example walking would be pieced together by paths from the
left foot in contact and paths with the right foot in contact.

\subsection{Speed Profile Path Space}

  \begin{equation}
    \begin{aligned}
      \PS(s) &= \{ \path \in \PSKE\ |\ s(\path): [0,T] \rightarrow [0,1]\}
    \end{aligned}
  \end{equation}

For dynamical systems like humanoid robots finding a speed profile with a convex
cost function is a convex optimization problem \cite{pham_2014} even under
contact constraints \cite{hauser_2013}.

%\section{Hierarchical Ordering}
%
%Using the structure we can define a hierarchical ordering 
%\footnote{
%  A binary relationship $a \le b $ between
%two objects is said to be a hierarchical ordering if there is a single root
%object $ r $ and: 
%
%For all $ a $, $ a \le a $ and $ r \le a $ and , If both
%$ a \le b $ and $ b \le a $ it follows that $ a = b $, The
%relationship is transitive: if $ a \le b $ and $ b \le c $, this
%implies that $ a \le c $, and If $ a \le c $ and $ b \le c $,
%this implies that either $ a \le b $ or $ b \le a $.
%
%
%Two objects $ a $ and $ b $ are said to be comparable if either
%$ a \le b $ or $ b \le a $; otherwise, they are said to be
%non-comparable.
%
%\url{https://ece.uwaterloo.ca/~dwharder/aads/Abstract_data_types/Hierarchical_ordering/}
%
%} on the path space.
%
%In particular, we define a set of equivalence relations on several spaces which
%in turn give us an ordering on the whole path space. 
%\begin{enumerate}
%  \item Equivalence relation on center of mass space. Two paths are equivalent
%    if they can be deformed into each other.
%  \item Equivalence relation 2 on center of mass space. Two paths are
%    equivalent, if we can deform them while sliding contacts along the
%    environment.
%\end{enumerate}
%
%

